Towards Diverse and Natural Image Descriptions via a Conditional GAN

Despite the substantial progress in recent years, the image captioning techniques are still far from being perfect.Sentences produced by existing methods, e.g. those based on RNNs, are often overly rigid and lacking in variability. This issue is related to a learning principle widely used in practice, that is, to maximize the likelihood of training samples. This principle encourages high resemblance to the "ground-truth" captions while suppressing other reasonable descriptions. Conventional evaluation metrics, e.g. BLEU and METEOR, also favor such restrictive methods. In this paper, we explore an alternative approach, with the aim to improve the naturalness and diversity -- two essential properties of human expression. Specifically, we propose a new framework based on Conditional Generative Adversarial Networks (CGAN), which jointly learns a generator to produce descriptions conditioned on images and an evaluator to assess how well a description fits the visual content. It is noteworthy that training a sequence generator is nontrivial. We overcome the difficulty by Policy Gradient, a strategy stemming from Reinforcement Learning, which allows the generator to receive early feedback along the way. We tested our method on two large datasets, where it performed competitively against real people in our user study and outperformed other methods on various tasks.

==> background.tex <==
% !TEX root = gantext_main.tex

\section{Background}
\label{sec:background}

Image description, a task to generate sentences to describe given
images, has been a active topic recently.
Many state-of-the-art frameworks~\cite{zhou2016image,you2016image,yang2016review,lu2016knowing,xu2015show,vinyals2015show} for this task adopt
the \emph{maximum likelihood} principle for learning.
%
Such a framework usually works as follows.
Given an image $I$, it first derives a feature representation $\vf(I)$,
and then generates the words $w_1, \ldots, w_T$ sequentially, following
a Markov process conditioned on $\vf(I)$.
%
The model parameters are learned via maximum likelihood estimation (MLE),
\ie~maximizing the conditional log-likelihood
of the training samples, as:
\begin{equation}
	\sum_{(I_i, S_i) \sim \cD}
	\sum_{t=0}^{T_i}
	\log p \left(w_i^{(t)} | \vf(I), w_i^{(t-1)}, \ldots, w_i^{(t-n)}\right).
\end{equation}
Here, $I_i$ and $S_i = (w_i^{(0)}, \ldots, w_i^{(T_i)})$ are the image and
the corresponding descriptive sentence of the $i$-th sample,
and $n$ is the order of the Markov chain
-- the distribution of the current work depends on $n$ preceding words.
%
Along with the popularity of deep neural networks, latest studies often
adopt neural networks for both image representation and language modeling.
For example, \cite{xu2015show} uses a CNN for deriving the visual features
$\vf(I)$, and an LSTM~\cite{hochreiter1997long}~to express the sequential relations among words.
%
Despite the evolution of the modeling choices, the maximum likelihood principle
remains the predominant learning principle.

% A trained model generates a sentence for a given image $I$ by sampling the words
% following the conditioned Markov chain.
As illustrated in Figure \ref{fig:mle_limit}, when similar images are presented,
the sentences generated by such a model often contain \emph{repeated} patterns.
This is not surprising -- under the MLE principle, the joint probability of a sentence
is, to a large extent, determined by whether it contains those n-grams that appear
frequently in the training set. Therefore, the model trained in this way will tend
to produce such n-grams. In particular, when the generator yield a couple of words
that match the prefix of a frequent n-grams, the remaining words of that
n-gram are very likely to be generated following the Markov chain.

% where it starts with an image $I$, and at each step it chooses a word that is
% most probable, which is ensured by the objective \ref{eq:mle_loss}. As shown in
% Figure \ref{fig:mle_limit}~(a), two trends can be observed in testing, (1) When
% it starts with unseen images $\{I\}$ that are slightly different but share large
% similarity to some seen image $I^\prime$, it is very likely to choose similar
% words for all these images $\{I\}$. (2) Besides that, when several consecutive
% choices of it meets a specific phrase which occurs frequently during training,
% it is very likely to choose a word that continues the phrase.

The quality of the generated sentences are usually assessed using
metrics originating from the machine translation area, such as
BLEU~\cite{papineni2002bleu}, ROUGE~\cite{lin2004rouge}, METEOR~\cite{lavie2014meteor}, and CIDEr~\cite{vedantam2015cider}.
Such metrics mostly rely on matching n-grams with the \emph{``ground-truths''}.
For example, the modified precision score $p$, which is the core
statistics in BLEU~\cite{papineni2002bleu}, is defined as
\begin{equation}
	p = \frac
	{\sum_{\omega \in \Omega} h_\text{clip}(\omega)}
	{\sum_{\omega^\prime \in \Omega} h(\omega^\prime)}.
\end{equation}
which basically counts the appearance of all n-grams in \emph{``ground-truths''} and generated sentences,
and computes their ratio.
As a result of the reliance of n-gram matching, sentences that contain frequent
n-grams will get good scores as compared to those using variant expressions,
as shown in Figure~\ref{fig:oldmetrics}.

Note that whereas image captioning is sometimes
considered as \emph{translating an image to a sentence}, it differs signficantly
from a conventional translation task, \eg~from English to Spanish.
When presented a photo, different people would probably give quite different
descriptions that do not overlap much in the wording patterns.
%
This diversity in expression is an essential property of human languages,
which, however, is often overlooked in previous work (both generation
and evaluation).
%
This study explores an alternative approach --
instead of emphasizing n-gram matching, we focus on improving the
\emph{naturalness}, \ie~generating sentences that feel like
what real people would say.


==> tab_paragen.tex <==
\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
	\toprule
	 			    & & BLEU-3 & BLEU-4 & METEOR & ROUGE\_L & CIDEr & SPICE & E-NGAN & E-GAN \\
	\midrule
	& G-MLE & \textbf{7.20} & \textbf{4.10} & \textbf{10.30} & \textbf{25.40} & \textbf{9.20} &  &  &  \\
	& G-GAN 			    &  &  &  &  &  &  &  &  \\
	\bottomrule
\end{tabular}
\caption{Results on paragraph generation. where we follow \cite{krause2016hierarchical} to multiple the results by $1,00$}.
\end{table*}

